Congestion-aware Ride-pooling in Mixed Traffic for Autonomous Mobility-on-Demand Systems

This paper presents a modeling and optimization framework to study congestion-aware ride-pooling Autonomous Mobility-on-Demand (AMoD) systems, whereby self-driving robotaxis are providing on-demand mobility, and users headed in the same direction share the same vehicle for part of their journey. Specifically, taking a mesoscopic time-invariant perspective and on the assumption of a large number of travel requests, we first cast the joint ride-pooling assignment and routing problem as a quadratic program that does not scale with the number of demands and can be solved with off-the-shelf convex solvers. Second, we compare the proposed approach with a significantly simpler decoupled formulation, whereby only the routing is performed in a congestion-aware fashion, whilst the ride-pooling assignment part is congestion-unaware. A case study of Sioux Falls reveals that such a simplification does not significantly alter the solution and that the decisive factor is indeed the congestion-aware routing. Finally, we solve the latter problem accounting for the presence of user-centered private vehicle users in a case study of Manhattan, NYC, characterizing the performance of the car-network as a function of AMoD penetration rate and percentage of pooled rides within it. Our results show that AMoD can significantly reduce congestion and travel times, but only if at least 40% of the users are willing to be pooled together. Otherwise, for higher AMoD penetration rates and low percentage of pooled rides, the effect of the additional rebalancing empty-vehicle trips can be even more detrimental than the benefits stemming from a centralized routing, worsening congestion and leading to an up to 15% higher average travel time.

==> Sections/Append.tex <==
% !TeX spellcheck = en_US
\appendices
\section{Proof of Lemma~\ref{lemma:finalprob}}\label{app:1}
%Since the two events are independent, to compute the probability of both happening \textcolor{blue}{within a time window $\bar{t}$}, \textcolor{blue}{one} can \textcolor{blue}{take the product of } multiply the probability of the two separate events and integrate it over the desired interval.

%the overall probability of the two events happening within a time interval $\bar{t}$ is the integral from $t=0$ to $t = \infty$ of one of the two functions, multiplied by the integral of the second function. However the extremes of the latter integral, are from $t-\bar{t}$ to $t-\bar{t}$.   

Recall that the exponential distribution, whose probability density function is given by $f(x)= \alpha e^{-\alpha x}$, models the time between events in a Poisson process of parameter $\alpha$. Since the two Poisson processes are independent,
\begin{equation*}
	\begin{split}
		P(\alpha_m,\alpha_n) = & \int_0^{\bar{t}} \alpha_n  e^{-\alpha_n  t_n} \left( \int_0^{t_n+\bar{t}} \alpha_m  e^{-\alpha_m t_m} \mathrm{d}t_m \right) \mathrm{d}t_n + \\
		& \int_{\bar{t}}^{\infty} \alpha_n e^{-\alpha_n t_n} \left(\int_{t_n-\bar{t}}^{t_n+\bar{t}} \alpha_m e^{-\alpha_m t_m}  \mathrm{d}t_m \right)  \mathrm{d}t_n,
	\end{split}
\end{equation*}
where the presence of two terms arises from the fact that the time interval $[0,+\infty)$ is considered. Making use of standard integral calculus techniques, it can be rewritten as \eqref{eq:lem}.
\begin{comment}
Evaluating the first integral we get
\begin{align*}
	\int_0^{\bar{t}} \int_0^{t_n+\bar{t}} \alpha_n   e^{-\alpha_n  t_n}  \alpha_m   e^{-\alpha_m  t_2}  \mathrm{d}t_2  \mathrm{d}t_n 
	%=\\ 
	%\int_0^{\bar{t}} \alpha_n  e^{-\alpha_n   t_n}  %\left(1 - e^{-\alpha_m   (t_n+\bar{t})}\right)  %\mathrm{d}t_n 
	=\\ 
	\int_0^{\bar{t}} \left( \alpha_n  e^{-\alpha_n   t_n} - \alpha_n  e^{-t_n \cdot(\alpha_n +\alpha_m) -\alpha_m   \bar{t}} \right)  \mathrm{d}t_n  
	=\\
	\left(1 - e^{-\alpha_n  \bar{t}}\right) - \frac{\alpha_n}{\alpha_n+\alpha_m} e^{-\alpha_m  \bar{t}}  \left(1 - e^{-(\alpha_n+\alpha_m) \bar{t}}\right),
\end{align*}
whilst from the second integral we obtain
\begin{align*}
	\int_{\bar{t}}^{\infty} \int_{t_n-\bar{t}}^{t_n+\bar{t}} \alpha_n e^{-\alpha_n  t_n}  \alpha_m  e^{-\alpha_m  t_2}  \mathrm{d}t_2  \mathrm{d}t_n 
	%=\\
	%\int_{\bar{t}}^{\infty} \alpha_n e^{-\alpha_n  t_n}  \left(e^{-\alpha_m  (t_n-\bar{t})} - e^{-\alpha_m  (t_n + \bar{t})}\right)   \mathrm{d}t_n 
	=\\ 
	\int_{\bar{t}}^{\infty} \alpha_n   e^{-(\alpha_n+\alpha_m)  t_n}   \left(e^{\alpha_m   \bar{t}}-e^{-\alpha_m   \bar{t}}\right)  \mathrm{d}t_n 
	=\\
	\frac{\alpha_n}{\alpha_n+\alpha_m}  \left(e^{\alpha_m   \bar{t}}-e^{-\alpha_m   \bar{t}}\right)  \left(e^{-(\alpha_n+\alpha_m) \bar{t}}\right).
\end{align*}
\end{comment}
%We obtain
\begin{comment}
\begin{align*}
	P_{kl} = 	\left(1 - e^{-\alpha_n  \bar{t}}\right) 
	-\\- \frac{\alpha_n}{\alpha_n+\alpha_m} e^{-\alpha_m  \bar{t}}  \left(1 - e^{-(\alpha_n+\alpha_m) \bar{t}}\right) 
	+\\+ 
	\frac{\alpha_n}{\alpha_n+\alpha_m}  \left(e^{\alpha_m   \bar{t}}-e^{-\alpha_m   \bar{t}}\right)  \left( e^{-(\alpha_n+\alpha_m) \bar{t}}\right) 
	=\\=
	\left(1 - e^{-\alpha_n  \bar{t}}\right) 
	-
	\frac{\alpha_n}{\alpha_n+\alpha_m} \cdot
	e^{-\alpha_m  \bar{t}}
	+\\+
	\frac{\alpha_n}{\alpha_n+\alpha_m}  e^{\alpha_m   \bar{t}}  \left(e^{-(\alpha_n+\alpha_m) \bar{t}}\right) 
	=\\=
	\end{align*}
\end{comment}
%\begin{align*}
%	P_{mn}(\alpha_m,\alpha_n) 
%	%&= 
%	%\left(1 - e^{-\alpha_n  \bar{t}}\right) - \frac{\alpha_n}{\alpha_n+\alpha_m}   \left(e^{-\alpha_m  \bar{t}} -  e^{-\alpha_n   \bar{t}}\right)\\
%	&= 1-\frac{\alpha_n e^{-\alpha_m\bar{t}}+\alpha_m e^{-\alpha_n\bar{t}}}{\alpha_n+\alpha_m}.
%\end{align*}
%We do a quick sanity check of the obtained results. If \mbox{$\alpha_n=0$} or $\alpha_m=0$, $P_{nm} =0$, meaning flows have 0\% probability of being matched. If $\alpha_n = \alpha_m$ the formula coincides with the original formulation with 1 event.

\section{Proof of Theorem~\ref{theorem:one}}\label{app:2}

%${\!\abs{\cM}(\abs{\cM}\!-\!1)\!}$ 

The convergence of Algorithm~\ref{alg:one} in at most ${\abs{\cM}(\abs{\cM}+1)/2}$ iterations is immediate. In fact, since for each pair $(m,n)$ chosen in each iteration we set $\Delta \tilde{J}^\prime_{mn} \!= \!\Delta \tilde{J}^\prime_{nm} \!= \!0$, neither $(n,m)$ nor $(m,n)$ will be chosen again. The optimality of the solution $\beta^\star$ and associated $\gamma^\star$ is carried out making use of an analogy with the . Recall that such algorithm consists in, every iteration, allocating the maximum amount of the resource with the highest improvement in the objective function per unit of  the resource, which is intuitively evident.  Similarly to the continuous Knapsack problem, the goal is to minimize $\tilde{J}(X^\star_\gamma)$ by allocating ${\gamma_{mn} \geq 0}$ with $m,n \in \cM$. First, borrowing the notation from Section~\ref{sec:SD}, if $\gamma_{mn}$ is assigned, then the corresponding decrease in the cost function amounts to $\tilde{J}(\gamma_{nm}X^{mn,0})\! -\!\tilde{J}(\gamma_{mn}X^{mn,\star}) =\gamma_{mn}(\tilde{J}(X^{mn,0})\! -\!\tilde{J}(X^{mn,\star})) = \gamma_{mn}\Delta{\tilde{J}}_{mn}$, where the linearity of $\tilde{J}$ played a key role. Thus, the allocation of $\gamma_{mn}$ leads to a relative improvement on the cost that amounts to $\Delta{\tilde{J}}_{mn}$. Second, as pointed out in Section~\ref{sec:alg}, throughout the algorithm, $\alpha^\prime_m$ corresponds to the demand of $r_m$ which has not yet been ride-pooled with another request. Thus, the value of $\gamma_{mn}$ that can be allocated has an upper bound given by $\gamma_{mn} \leq \min(\alpha_m^\prime, \alpha_n^\prime)P(\alpha_m^\prime,\alpha_n^\prime)$. Note that Algorithm~\ref{alg:one} corresponds to allocating the maximum amount of $\gamma_{mn}$, where $m$ and $n$ are such that, at each iteration, the highest positive relative improvement in the objective function is achieved, i.e., $(m,n) \in \mathrm{argmax}_{m,n} (\Delta \tilde{J}^\prime_{mn})$, which shows its optimality.




%We prove Theorem~\ref{theorem:one} by contradiction. If $\beta$ would not be an optimal parameter, there would exist an optimal parameter $\beta'$, so that the objective of Problem~\ref{prob:rides} $\tilde{J}(X^\star_{\gamma'}) < J(X^\star_{\gamma})$, where $X^\star_{\gamma}$ is the optimal solution of Problem~\ref{prob:rides} with demand matrix $D^\mathrm{rp}$, that, leveraging~\eqref{eq:b}, is a function of the expected number of pooled rides $\gamma$, that in turn is a function of the assignment matrix $\beta$.  To have a more compact notation, we define $\gamma_{nm}=\gamma_{nm}(\beta_{nm},\beta_{mn})$, and $\gamma'_{nm}=\gamma_{nm}(\beta'_{nm},\beta'_{mn})$. Moreover, we define $\Delta J _{nm} = \Delta J _{nm}(X^\star_{\gamma_{nm}})$, $\Delta J'_{nm} = \Delta J_{nm}(X^\star_{\gamma'_{nm}})$, and $\Delta J_{nm}^1 = \Delta J_{nm}(X^\star_{D^{nm,\star}})$.
%We recall that $ \Delta J _{nm}(X^\star_{\gamma_{nm}})$ is linear w.r.t. $\gamma_{nm}$. In turn, $\gamma_{nm}$ is monotonically increasing w.r.t. $\beta_{nm}$ and $\beta_{mn}$.
%For the sake of simplicity, let's consider a simple case with only 2 demands $n$ and $m$. They can both pool with themselves---pooling options $nn$ and $mm$---and with the other one---pooling options $nm$ and $mn$---. The algorithm prioritizes the pooling of a requests with the highest improvement in the partial objective function. In this case, options $nn$ and $mm$ will be prioritized because they have no delay.
%This results in
%\begin{equation}\label{eq:lin2}
%	\Delta J^1 _{nm} < \Delta J^1 _{mm}, \;\; \Delta J^1_{mn} < \Delta J^1_{mm},
%\end{equation} 
%\begin{equation*}
%	\Delta J^1_{nm} < \Delta J^1 _{nn}, \;\; 	\Delta J^1_{mn} < \Delta J^1 _{nn}. 
%\end{equation*}
%If $\beta$ is not the optimal parameter, then $\beta'$ would exist so that:
%\begin{equation} \label{eq:monot}
%	\beta_{nn} - \beta'_{nn}  \geq 0, \;\;\beta_{nm} - \beta'_{nm} \leq 0,
%\end{equation} 
%\begin{equation*}
%	\beta_{mm} -  \beta'_{mm} \geq 0, \;\; 	\beta_{mn} - \beta'_{mn} \leq 0.
%\end{equation*} 
%Since travel time is constant, it follows that
%\begin{equation}
%	\Delta J_{nn}+ \Delta J_{mm} + \Delta J_{nm} + \Delta J_{mn} <  
%\end{equation}
%\begin{equation*}
%	< \Delta J'_{nn} + \Delta J'_{mm}+ \Delta J'_{nm} + \Delta J'_{mn}. 
%\end{equation*}
%The problem linear in $\gamma$. It means that \begin{equation}\label{eq:deltaj}
%	(\gamma_{nn} -\gamma'_{nn} )\Delta J^1_{nn} +
%  (\gamma_{mm} -\gamma'_{mm} )\Delta J^1_{mm} -
%\end{equation}
%\begin{equation*}
%	-(\gamma_{nm} -\gamma'_{nm} )\Delta J^1_{nm}- (\gamma_{mn} -\gamma'_{mn} )\Delta J^1_{mn} < 0.
%\end{equation*}
%By leveraging Eq.~\eqref{eq:lin2},\eqref{eq:monot} and recalling that $\gamma$ is monotone w.r.t. $\beta$, Eq.~\eqref{eq:deltaj} never holds, resulting in $J(X^\star_{\gamma'}) \geq J(X^\star_{\gamma})$.  This concludes the proof.

==> Sections/Model.tex <==
% !TeX spellcheck = en_US


\subsection{Ride-pooling Time-invariant Network Flow Model}

Recently, in \cite{PaparellaPedrosoEtAl2023}, the authors proposed a formulation to take into account ride-pooling without the need to change the original structure of the problem. We transform the original set of requests, portrayed by $D$, into an equivalent set of requests accounting for ride-pooling, portrayed by $D^\mathrm{rp}$. We define the ride-pooling network flow problem as follows:
\begin{prob}[Ride-pooling Network Flow Problem]\label{prob:rides}
	Given a road graph $\cG$ and a demand matrix $D^\mathrm{rp}$, the active vehicle flows $X$ and rebalancing flow $x^\mathrm{r}$ that minimize the cost in terms of overall travel time result from
	\begin{equation*}
		\begin{aligned}
			\min_{X,x^\mathrm{r}}\; &J(X,x^\mathrm{r}) = {t(X,x^\mathrm{r})^\top (X \mathds{1} + \rho x^\mathrm{r})} \\
			\mathrm{s.t. }\; & BX = D^\mathrm{rp} \\
			&B ( X \mathds{1}+ x^\mathrm{r} )= 0 \\
			& X, x^\mathrm{r} \geq 0.
		\end{aligned}
	\end{equation*}
\end{prob}

The ride-pooling demand matrix $ D^\mathrm{rp}$ in Problem~\ref{prob:rides} describes the pooling pattern, i.e., how the different request are allocated to be pooled (or not) together. In particular, four key conditions must be met, which are thoroughly detailed and analyzed in \cite{PaparellaPedrosoEtAl2023}. First, all the individual requests, described by $D$, must be served. Second, ride-pooling two requests is only spatially feasible if the detour travel time of both requests is not greater than a threshold $\bar{\delta} \in \mathbb{R}_{ \geq 0}$. Third, ride-pooling two requests is only temporally feasible if the waiting time for a request to start being served does not exceed a threshold $\bar{t} \in \mathbb{R}_{>0}$. Fourth, the requests are pooled to minimize the cost function of Problem~\ref{prob:rides} at its solution. 

\subsection{Congestion-unaware approach}

In \cite{PaparellaPedrosoEtAl2023}, the authors proposed an approach to optimally compute the ride-pooling demand matrix $D^\mathrm{rp}$ for $\rho = 0$ in a congestion-unaware setting, i.e., assuming the arc travel times are constant. Then Problem~\ref{prob:rides} could be solved for the flows under the congestion-unaware assumption. Notwithstanding the combinatorial nature of matching rides, this approach supported on the network flow formulation, allowed to attain a computationally tractable polynomial-time algorithm.

However, it is not possible to extend this approach to a congestion aware 


\subsection{Discussion}

A few comments are in order. First, the mobility system is analyzed at steady-state in a time-invariant framework, which is unsuitable for an online implementation, but it has been used for planning and design purposes by several works in the literature as seen in Section~1. This assumption is reasonable if the travel requests vary slowly w.r.t. the average time of serving each request. This is the case especially in highly populated metropolitan areas \cite{IglesiasRossiEtAl2017}. Second, our framework does not take into account the stochastic nature of the exogenous congestion that determines that travel time in each road arc. However, this deterministic approach is suitable for our purposes as it provides an average representation of these stochastic phenomena in a mesoscopic scale \cite{Neuburger1971}. Third, Problems~\ref{prob:main} and \ref{prob:rides} allow for fractional flows, which is acceptable because of the mesoscopic perspective of the work~\cite{PaparellaChauhanEtAl2023,LukeSalazarEtAl2021,SalazarLanzettiEtAl2019}. Finally, $D^\mathrm{rp}$ is not optimal w.r.t. the objective function of Problem~\ref{prob:rides}, but it is w.r.t. its relaxed version, enabling a polynomial-time computation.


\begin{approximation}\label{approx}
For the purpose of computing the demand matrix $D^\mathrm{rp}$,  the cost function of Problem~\ref{prob:rides} is set for $\rho = 0$, i.e., $\tilde{J_1}(X,x^\mathrm{r}):=t(X,x^\mathrm{r})^\top X \mathds{1}$.
\end{approximation}
It is crucial to remark that this approximation is only employed in a first step to compute $D^\mathrm{rp}$ and, afterwards, in a second stage, the passenger and rebalancing flows are optimized jointly according to Problem~\ref{prob:rides}. This is in order for an Autonomous Mobility on Demand fleet, for example, which is centrally operated and whose vehicles do not compete for rides.
This is a very common approximation used in the literature \cite{Alonso_Mora_2017}, which is leveraged to devise a polynomial-time algorithm to compute $D^\mathrm{rp}$ that is optimal w.r.t. the version of the problem with $\rho=0$. In the following, the essential steps are highlighted. We refer the readers to ~\cite{PaparellaPedrosoEtAl2023} for a detailed description of the approach.  

Compared to~\cite{PaparellaPedrosoEtAl2023}, the objective is still a function of $x^\mathrm{r}$, even for $\rho =0$. To this end, we leverage the findings in~\mbox{\cite[Ch.3.3.2]{Rossi2018}} to recall that assuming there exists a feasible customer flow, it is
always possible to find a feasible rebalancing flow.
Hence we modify Approximation~\ref{approx} accordingly.
\begin{approximation}\label{approx2}
	$\tilde{J}(X):=t(X)^\top X \mathds{1}$.
\end{approximation} 



\subsection{Approximate  Computation of the Demand Matrix}

In this section, we present a framework to compute the demand matrix $D^\mathrm{rp}$ under Approximation~\ref{approx}.  

% we ormalize the four conditions and present a alg which is optimal in relation to j tilde


\begin{comment}
\subsubsection{Spatial Analysis of Ride-pooling}\label{sec:SD}
%TO BE ADDED BEFORE THE TIME|SPACE sections\msmargin{In a ride pooling environment, both space and time are relevant to understand if \textcolor{blue}{two} requests can be pooled. However, in Problem~\ref{prob:main}, the elements of the OD matrix $b$ are coefficients of a Poisson process (i.e., \textcolor{blue}{it models} requests per unit time). For this reason, we must move from a deterministic point of view to a probabilistic one. In particular, we decouple time properties of the requests from the spacial ones: We first compute the optimal ride pooling paths, and then, we evaluate the probability of them happening. We define the following ride pooling problem.}{dobbiamo rendere questo paragrafo pi\`u chiaro: \`e cruciale per il paper}
In this section, we analyze the feasibility and optimal configuration of ride-pooling two requests from a spatial perspective. First, we define $\delta$ as the delay experienced by each user, representing the time required to travel the additional detour distance w.r.t. the scenario without ride-pooling. If the delay experienced by any of the two users is higher than the threshold $\bar{\delta}$, then pooling the two requests is unfeasible. Second, 
given the feasible pooling itineraries, we analyze which one is the optimal, i.e., the best itinerary to serve the requests, and whether pooling is advantageous w.r.t. no pooling.
Consider two requests $r_m,r_n\in \cR$. To restrict this analysis to the spatial dimension, we temporarily make two key considerations, that we lift in Section~\ref{sec:STF}: i)~the requests $r_m$ and $r_n$ are made at the same time; and ii)~both requests have the same demand, which we set, without any loss of generality, to $\alpha=1$. %$\alpha \in \mathbb{R}^+$.
\begin{figure}[t]
	\centering
	\includegraphics[width = 0.65\linewidth]{Figures/serve_conf-eps-converted-to.pdf}
	\caption{Distinct configurations for serving two requests $r_m,r_n \in \cR$. Each arrow represents a flow of $\alpha = 1$ vehicles. The dashed arrows represent a flow with two users, whilst the solid ones represent a flow with one user.}
	\label{fig:serve_conf}
	\vspace{-0.5cm}
\end{figure}
There are five different ways of serving two requests $r_m, r_n \in \cR$, as depicted in Fig.~\ref{fig:serve_conf}.
The goal is to assess whether it is feasible to ride-pool $r_m$ and $r_n$ and which is the best configurations among the five. Index each configuration with number $c \in \{0,\ldots,4\}$, with $c=0$ corresponding to no pooling. Each configuration can be split into either two or three equivalent travel requests, as shown in Fig.~\ref{fig:serve_conf}, each corresponding to an arrow. Denote the set of such equivalent requests for configuration $c$ as $\cR_{mn}^c$ ($\cR_{nm}^c = \cR_{mn}^c$) and we define $\Pi(\cR_{mn}^c)$ as the order of visited nodes. For each configuration $c$, one can now solve Problem~\ref{prob:rides}, under Approximation~\ref{approx},  with a simplified demand matrix $D^\mathrm{rp} = D^{mn,c}$ obtained from the set of requests $\cR_{mn}^c$ with \eqref{eq:def_D}, obtaining a flow $X^{mn,c} \in \mathbb{R}^{\abs{\mathcal{V}}\times \abs{\mathcal{V}}}$. %From the flows for each configuration, $X^c, c \in \{0,\ldots,4\}$, the questions that we set out to answer in this subsection follow immediately. 
The delay $\delta^{m,c}$ of request $r_m$ for a configuration $c$, is
\begin{equation*}
	\delta^{m,c} = \sum_{p \in {\pi^c_{mn}} } [t^\top X^{mn,c}]_p   - [t^\top X^{mn,0}]_{o_m},
\end{equation*}
where ${\pi^c_{mn}} \subseteq \Pi(\cR_{mn}^c)$ is the ordered set of nodes $\Pi(\cR_{mn}^c)$ from $o_m$ to the node before $d_m$. 
The feasible configurations are those whose delay of both users is below the threshold $\bar{\delta}$. Then, among the feasible ones, comprehending also the no pooling option, the optimal configuration is the one whose flow $X^{mn,c}$ achieves the lowest cost $\tilde{J}(X^{mn,\star})$. Henceforth, the simplified demand matrix of the optimal configuration for ride-pooling $r_m$ and $r_n$ is denoted by $D^{mn,\star}$.

% Before revision 
%\begin{remark} The demand matrix $D^{mn,c}$ contains either two or three equivalent travel requests. To reduce the computational load, Problem~\ref{prob:rides} can be computed for each equivalent request and stored separately. It amounts to solve Problem~\ref{prob:rides} $\abs{\cV}^2$ times. Since each has a computational complexity of $\mathcal{O} (\abs{\cV}^2)$, the overall computational complexity is $\mathcal{O} (\abs{\cV}^4)$. The procedure depends on the graph $\mathcal{G}$, meaning that the computations have to be performed only once.
%\end{remark}

% After revision
\begin{remark} The demand matrix $D^{mn,c}$ contains either two or three equivalent travel requests between the origin and destination nodes of requests $r_m$ and $r_n$. To reduce the computational load, a graph search technique can be employed instead, to compute the shortest path between every pair of nodes. Since each instance has a worst-case computational complexity of $\mathcal{O} (\abs{\cV}^2)$, the overall computational complexity is $\mathcal{O} (\abs{\cV}^4)$. The procedure depends on the graph $\mathcal{G}$, meaning that the computations have to be performed only once.
\end{remark}
\begin{remark}
The procedure can be extended to account for the possibility of pooling three or more requests. In this case, the number of possible configurations increases \rev{in a combinatorial trend}, but \rev{since the number of requests that is possible to ride-pool is limited}, the overall \rev{asymptotic} complexity remains $\mathcal{O} (|\mathcal{V}|^4)$.
%The procedure can be extended to account for the possibility of pooling three or more requests. In this case, the number of possible configurations increases, but the overall complexity remains $\mathcal{O} (\abs{\cV}^4)$.
\end{remark}
\end{comment}

==> Sections/Model0.tex <==
% !TeX spellcheck = en_US

\section{Ride-pooling Network Flow Model}\label{sec:model}

In this section, we introduce the network  traffic flow model~\cite{PavoneSmithEtAl2012}. Then, we extend it to take into account ride-pooling, and finally present a brief discussion on the model.

%From the vehicle flows can then be reconstructed  reconstruct 

% \rev{Leveraging flow decomposition algorithms \cite{AhujaMagnantiEtAl1993}, the microscopic vehicle routes can be reconstructed}

\subsection{Time-invariant Network Flow Model} 
% Note ref: PaparellaChauhanEtAl2023 is broken, it is not on the bib anaymore (add to the first cite later PaparellaChauhanEtAl2023)
We model the mobility system as a multi-commodity network flow model, similar to the approaches of~\cite{SalazarLanzettiEtAl2019,LukeSalazarEtAl2021,PaparellaChauhanEtAl2023,RossiIglesiasEtAl2018b,PaparellaSripanhaEtAl2022}. The transportation network is a directed graph $\mathcal{G} = (\mathcal{V}, \mathcal{A})$. {It consists of a set of vertices $\mathcal{V} := \{1,2,...,\abs{\mathcal{V}}\}$,} representing the location of intersections on the road network, and {a set of arcs $\mathcal{A} \subseteq \mathcal{V} \times \mathcal{V}$}, representing the road links between {intersections}. We indicate ${B \in \{-1,0,1\}^{\abs{\cV} \times \abs{\cA}}}$ as the incidence matrix~\cite{Bullo2018} of the road network $\mathcal{G}$. Consider an arbitrary arc indexing of natural numbers $\{1,\ldots,\abs{\cA}\}$, then $B_{ip} = -1$ if the arc indexed by $p$ is directed towards vertex $i$, $B_{ip} = 1$ if the arc indexed by $p$ leaves vertex $i$,  and $B_{ip}=0$ otherwise. Similarly to \cite{PavoneSmithEtAl2012}, we define travel requests as follows:
\begin{definition}[Requests]
	A travel request is defined as the tuple $r = (o,d,\alpha) \in \mathcal{V} \times \mathcal{V} \times \mathbb{R}_{>0}$, in which $\alpha$ is the number of users traveling from the origin $o$ to the destination $d \neq o$ per unit time.  Define the set of requests as $\mathcal{R} := \{r_m\}_{m\in \mathcal{M}}$, where $\mathcal{M} = \{1,\ldots,M\}$.
\end{definition} 

We assume, without any loss of generality, that the origin-destination pairs of the requests $r_m \in \mathcal{R}$ are distinct. 
In this paper, we distinguish between active vehicle flows, which correspond to the flows of vehicles serving users whether they are ride-pooling or not, and rebalancing flows which correspond to the flows of empty vehicles between the drop-off and pick-up vertices of consecutive requests. We define the active vehicle flow induced by all the requests that share the same origin $i \in {\mathcal{V}}$ as vector $x^{i}$, where element $x^{i}_{a}$ is the flow on arc $a \in \cA$, ordered in accordance with the arc ordering of $B$. The overall active vehicle flow is a {matrix $X \in \mathbb{R}^{\abs{\cA} \times \abs{\cV}}$ defined as $X := \left[x^{1}\  x^2 \, \dots \,x^{\abs{\cV}}\right]$}. The rebalancing flow across the arcs is denoted by $x^{\mathrm{r}} \in \mathbb{R}^{\abs{\cA}}$. We denote $t(X,x^r)$ as the vector whose entries are the travel time $t_{a}$ required to traverse each arc $a\in \cA$, ordered in accordance with the arc ordering of $B$, which is a function of the active vehicle flows and rebalancing flows on that arc.  In the following, we define the network flow problem.
\begin{prob}[Multi-commodity Network Flow Problem]\label{prob:main}
	Given a road graph $\cG$ and a set of travel requests $\cR$, the active vehicle flows $X$ and rebalancing flow $x^\mathrm{r}$ that minimize the cost in terms of overall travel time result from
	\begin{equation*}
		\begin{aligned}
			\min_{X, x^\mathrm{r}}\; &J(X,x^\mathrm{r}) =t(X,x^r)^\top ( X \mathds{1} + \rho x^\mathrm{r} )  \\
			\mathrm{s.t. }\; & BX = D \\
			&B ( X \mathds{1}+ x^\mathrm{r} )=0 \\
			& X, x^\mathrm{r} \geq 0,
		\end{aligned}
	\end{equation*}
where $\rho \in [0;1]$ is a weight, and the demand matrix $D \in \mathbb{R}^{\abs{\mathcal{V}} \times \abs{\mathcal{V}}}$ represents the requests between every pair of vertices, whose entries are
	\begin{equation}\label{eq:def_D}
		\!\!\!\!D_{ij} = \begin{cases}
			\alpha_m, &  \exists m \in \mathcal{M} : o_m = j \land d_m = i\\
			-\sum_{k\neq j} D_{kj}, & i  = j \\ %\sum \limits_{\substack{k = 1 \\ k\neq i}}^{\abs{\mathcal{V}}} D_{ik}
			0, &   \mathrm{otherwise}.%i\neq j \land \nexists m \in \mathcal{M} : o_m = i \land d_m = j\\
		\end{cases}\!\!\!
	\end{equation}
\end{prob}
%Problem~\ref{prob:main} is totally unimodular only for $\rho =0$. In that case the objective function is the minimum user travel time and $X$ and $x^\mathrm{r}$ can be decoupled and  computed separately~\cite{Rossi2018}. 
For $\rho =1$ the objective function, that represents the overall travel time of the fleet, can also be interpreted as the minimum fleet size required to implement the flows~\cite{PavoneSmithEtAl2012,Rossi2018}. For $\rho =0$ the objective function is the minimum user travel time.



%  




==> Sections/Model2.tex <==
% !TeX spellcheck = en_US
\begin{comment}
\subsubsection{Temporal Analysis of Ride-pooling}\label{sec:TD}
In this section, we analyze the temporal alignment of two requests for ride-pooling.  %Specifically, we define $\bar{t}$ as the maximum waiting time since the event of a request and the event of starting to serve that request. 
We derive the probability of two requests taking place within the maximum waiting time, $\bar{t}$. As common in traffic flow models~\cite{PavoneSmithEtAl2012}, we consider that the arrival rate of a request $r_m \in \cR$ follows a Poisson process with parameter $\alpha_m$. Consider two requests $r_m, r_n \in \cR$. In the following lemma, we indicate the probability of %being possible to ride-pool those requests in a temporal perspective, i.e., the probability of 
the two events occurring within a maximum time window $\bar{t}$.
%Note that we consider that a request which can be ride-pooled starts being served when the ride-poolling configuration starts, no matter its origin node.
%%In this second part, we show the \msmargin{mathematical formulation to compute the probability}{why?} of two events (the OD pairs) happening within a maximum waiting time, $\bar{t}$. 
%
%In traffic flow models~\cite{PavoneSmithEtAl2012}, the arrival rate of a request follows a Poisson process with parameter $\alpha$.
%\msmargin{We consider two events 1 and 2 with parameters $\alpha_1,\alpha_2$. It has to be computed the probability that, within a maximum time window, one occurrence of each event happens so that they are matched together for pooling. }{unclear}
%We announce the following lemma, that we prove in Appendix 2.
\begin{lemma}\label{lemma:finalprob}
Let $r_m, r_n \in \cR$ be two requests whose arrival rate follow a Poisson process with parameters $\alpha_m$ and $\alpha_n$, respectively. The probability of each having an occurrence within a maximum time interval $\bar{t}$ is
\begin{equation}\label{eq:lem}
	P(\alpha_m,\alpha_n)  := 1-\frac{\alpha_m e^{-\alpha_n\bar{t}}+\alpha_n e^{-\alpha_m\bar{t}}}{\alpha_m+\alpha_n}.
\end{equation}
\end{lemma}
\begin{proof}
	The proof can be found in Appendix~\ref{app:1}.
\end{proof}
\end{comment}
\subsubsection{Expected Number of Pooled Rides}%Stochastic Assignment in Ride-pooling} 
\label{sec:STF}
%In Section~\ref{sec:SD}, we analyzed the spatial dimension of the ride-pooling problem, whereby we computed the best feasible pooling path given two requests. In Section~\ref{sec:TD}, we analyzed the temporal dimension of the ride-polling problem, whereby we derived the probability of two requests happening within a time window.  By lifting the temporary assumptions made in Section~\ref{sec:SD}, we formulate the ride-pooling demand matrix given a certain pooling assignment, defined in what follows.

A fraction of the demand of every request $r_m\in \cR$ can be assigned to be pooled with a request $r_n \in \cR$. Let ${\beta \in \mathbb{R}_{\geq0}^{|\cR|\times |\cR|}}$ denote the assignment matrix, whose entry $(m,n)$ is the demand of $r_m$ that is assigned to be pooled with $r_n$. %Matrix $\beta$ defines the ride-pooling assignment. 
For the remainder of this subsection we assume that $\beta$ is given. In Section~\ref{sec:alg}, we propose an algorithm to compute the optimal value of $\beta$ under Approximation~\ref{approx}.

Only a fraction of the allocated ride-pooling demand $\beta_{mn}$ can actually be pooled due to temporal constraints. Specifically, the probability of pooling is given by $P(\beta_{mn},\beta_{nm})$ according to the following Lemma. 
\begin{lemma}\label{lemma:finalprob}
	Let $r_m, r_n \in \cR$ be two requests whose arrival rate follow a Poisson process with parameters $\alpha_m$ and $\alpha_n$, respectively. The probability of each having an occurrence within a maximum time interval $\bar{t}$ is
	\begin{equation}\label{eq:lem}
		P(\alpha_m,\alpha_n)  := 1-\frac{\alpha_m e^{-\alpha_n\bar{t}}+\alpha_n e^{-\alpha_m\bar{t}}}{\alpha_m+\alpha_n}.
	\end{equation}
\end{lemma}
Moreover, given that we only consider pooling between two requests, at most, the maximum pooled demand between $r_m,r_n\in \cR$ is  $\min(\beta_{mn},\beta_{nm})$. Therefore, the effective expected pooled demand between two requests $r_m,r_n\in \cR$ is given by ${\gamma_{nm} = \gamma_{mn} := \min(\beta_{mn},\beta_{nm})P(\beta_{mn},\beta_{nm})}$.  As a result, this pooled demand is portrayed by the demand matrix $\gamma_{mn}D^{mn,\star}$, where $D^{mn,\star}$ is the demand matrix of the optimal configuration for ride-pooling $r_m$ and $r_n$, i.e., the best serving order. The optimal configuration is the one whose flow $X^{mn,c}$ achieves the lowest cost $\tilde{J}(X^{mn,\star})$. Note that the effective expected pooling demand follows $\sum_{n\in \cM} \gamma_{mn} \leq \alpha_m, \, \forall r_m \in \mathcal{R}$ with equality if the full demand of $r_m$ is pooled.
The full ride-pooling demand matrix $D^\mathrm{rp}$ is made up of two contributions: i)~the sum of the expected pooled active vehicle flows of the form $\gamma_{mn}D^{mn,\star}$ for ${r_m,r_n\in \cR}$; and ii)~the requested demands that were not ride-pooled. Thus, the entry $(i,j)$ of $D^\mathrm{rp}$ can be written as
\begin{equation*}\label{eq:b}
		\!D_{ij}^{\mathrm{rp}} = \begin{cases}
			\sum\limits_{\substack{p,q\in \cM\\ p\geq q}} \gamma_{pq}D_{ij}^{pq,\star} + \left(D_{ij} - \sum\limits_{p\in\cM}\gamma_{mp}D_{ij}^{mp,\star} \right), \\ 
			 \quad \quad  \quad \quad  \quad \quad  \quad \quad \;\; \exists m \in \mathcal{M} : d_m \!= i \land o_m\! = j\\
			- \sum_{k\neq j} D_{kj}^{\mathrm{rp}},  \quad \quad \quad  i  = j \\ %\sum \limits_{\substack{k = 1 \\ k\neq i}}^{\abs{\mathcal{V}}} D_{ik}
				\sum\limits_{\substack{p,q\in \cM\\ p\geq q}} \gamma_{pq}D_{ij}^{pq,\star}, \quad \quad   \text{otherwise}.%i\neq j \land \nexists m \in \mathcal{M} : o_m = i \land d_m = j\\
		\end{cases}
\end{equation*}
However, because of the congestion-aware settings, the optimal flows and the matrix are a function of all the flows $X,x^\mathrm{r}$.

Hence, a method to solve this problem is using fixed-point iterations: an initial guess of $D^\mathrm{rp}$ is used as input in Problem~\ref{prob:rides}, which yields an LP, given a pooling assignment $\beta$. Then, the resulting flows are used as new inputs for the next computation of $D^\mathrm{rp}$. The process is repeated until a given convergence criterion is met.  

==> Sections/Model3.tex <==
% !TeX spellcheck = en_US


\subsubsection{Optimal Ride-pooling Assignment}\label{sec:alg}
In this section, given an initial level of road congestion, we will compute the optimal ride-pooling assignment matrices $\beta^\star$ and $\gamma^\star$, under Approximation~\ref{approx2}. We employ the same method used to solve the continuous Knapsack problem, which can be solved by a well-known polynomial-time greedy algorithm~\cite{Dantzig1957}.
For every pair of requests $r_m,r_n\in \cR$, we can compute the unitary improvement of the objective function of Problem~\ref{prob:rides}, denoted by $\Delta \tilde{J}_{mn}$, w.r.t. the no-pooling scenario. Specifically, it amounts to the difference  between $\tilde{J}_{nm}$, which denotes the cost with $D^\mathrm{rp} = D^{mn,\star}$, and $\tilde{J}_n+\tilde{J}_m$, which again denotes the cost with $D^\mathrm{rp} = D^{mn,0}$. Let $\alpha_m^\prime, m\in \cM$ stand for an auxiliary variable throughout the iterations and represent the demand of request $r_m$ that has not yet been assigned, and which is initialized as $\alpha_m^\prime = \alpha_m$. Further, the pair of requests with the highest improvement is prioritized with the highest possible pooling demand assignment. That is, in each iteration, if $r_m,r_n\in \cR$  is the pair of requests with the highest $\Delta \tilde{J}_{mn}$, we set $\beta_{mn} = \alpha_m^\prime$ and $\beta_{nm}=\alpha_n^\prime$. Moreover, the rides that have been assigned but not pooled, are added back to the original requests, i.e., we set $\alpha_m^\prime =  \beta_{mn}-\gamma_{mn}$ and $\alpha_n^\prime =\beta_{nm}-\gamma_{nm}$. Let $\Delta \tilde{J}_{mn}^\prime, m,n\in \cM$ denote another auxiliary variable  throughout the iterations, initialized as $\Delta \tilde{J}_{mn}^\prime=  \Delta \tilde{J}_{mn}$. At the end of every iteration, $\Delta \tilde{J}^\prime_{mn}$ is set to  0.   
This procedure is repeated until convergence is achieved, i.e., $\max_{m,n} (\Delta \tilde{J}^\prime_{mn}) \leq 0$. The pseudocode of this procedure is presented in Algorithm~\ref{alg:one}.
	
\begin{algorithm}[ht]
	\caption{Compute optimal assignment matrices $\beta^\star, \gamma^\star$.}\label{alg:one}
	\begin{algorithmic}
		\STATE $\tilde{J}_{mn} \leftarrow  \mathrm{input} \;\; D^{mn, \star} \; \text{to Problem}~\ref{prob:rides}, \;\; \forall {m,n\in \cM}$
		\STATE $\tilde{J}_{m} + \tilde{J}_n  \leftarrow  \mathrm{input} \;\; D^{mn, 0} \; \text{to Problem}~\ref{prob:rides}, \;\; \forall {{m,n\in \cM}}$
%		\STATE $ \forall m,n \; \mathrm{input} \; D^{mn,0} \; to \; Problem~\ref{prob:rides} \rightarrow \tilde{J}_{m},\tilde{J}_{n}$
		\STATE $\Delta \tilde{J}_{mn} \;\leftarrow\; \tilde{J}_{m} + \tilde{J}_{n} - \tilde{J}_{mn} $
		\STATE $\Delta \tilde{J}_{mn}^\prime \;\leftarrow\; \Delta \tilde{J}_{mn}, \; \forall m,n\in \cM$
		\STATE $\alpha_{m}^\prime \;\leftarrow\; \alpha_{m}, \; \forall m\in \cM $
%		\STATE $\;D^\mathrm{rp} = \mathbb{0}$
		\WHILE {$ \mathrm{max}_{m,n}(\Delta \tilde{J}^\prime_{mn}) > 0 $}
		\STATE $ (m,n) \in \mathrm{argmax}_{m,n} (\Delta \tilde{J}^\prime_{mn})$
		\IF{$o_n = o_m \; \mathrm{and} \; d_n=d_m$}
		\STATE $ \beta_{mn}  \;\leftarrow\; \alpha_{m}^\prime, \;\beta_{nm} \;\leftarrow\; \beta_{mn}$
		\STATE $ \gamma_{mn} \;\leftarrow\; \beta_{mn}  P(\beta_{mn},\beta_{nm})/2, \;\gamma_{nm} \;\leftarrow\; \gamma_{mn}$
%		\STATE $D^\mathrm{rp}_{ii} = b^\mathrm{rp}_{ii} - \beta_{ijkl} , \; b^\mathrm{rp}_{ij} = b^\mathrm{rp}_{ij} + \beta_{ijkl}  $
		\ELSE
		\STATE $\beta_{nm}  \;\leftarrow\;  \alpha_{n}^\prime, \; \beta_{mn}  \;\leftarrow\;  \alpha_{m}^\prime$
		\STATE $\gamma_{mn}  \;\leftarrow\;  \min(\beta_{nm},\beta_{mn}) P(\beta_{mn},\beta_{nm})$
		\STATE $\gamma_{nm} \;\leftarrow\;  \gamma_{mn}$
		\ENDIF
%		\STATE $D^\mathrm{rp} = D^\mathrm{rp} + \gamma_{mn}  D^{mn \star}$
		\STATE$\alpha_{m}^\prime  \;\leftarrow\;  \alpha_{m}^\prime - \gamma_{mn},  \; \alpha_{n}^\prime  \;\leftarrow\; \alpha_{n}^\prime - \gamma_{nm} $
		\STATE$\Delta \tilde{J}^\prime_{mn}  \;\leftarrow\; 0, \;   \Delta \tilde{J}^\prime_{nm} \leftarrow \Delta \tilde{J}^\prime _{mn}  $
		\ENDWHILE
	\end{algorithmic}
\end{algorithm}

\subsection{Fixed-point Iteration}
In the previous sections we explained how to compute the optimal assignment matrices $\beta^\star,\gamma^\star$ given a road congestion level. In this section we devise a fixed-point iteration method to compute the real congestion level at which the matrices have to be computed.
\subsection{Discussion}

A few comments are in order. First, the mobility system is analyzed at steady-state in a time-invariant framework, which is unsuitable for an online implementation, but it has been used for planning and design purposes by several works in the literature as seen in Section~1. This assumption is reasonable if the travel requests vary slowly w.r.t. the average time of serving each request. This is the case especially in highly populated metropolitan areas \cite{IglesiasRossiEtAl2017}. Second, our framework does not take into account the stochastic nature of the exogenous congestion that determines that travel time in each road arc. However, this deterministic approach is suitable for our purposes as it provides an average representation of these stochastic phenomena in a mesoscopic scale \cite{Neuburger1971}. Third, Problems~\ref{prob:main} and \ref{prob:rides} allow for fractional flows, which is acceptable because of the mesoscopic perspective of the work~\cite{PaparellaChauhanEtAl2023,LukeSalazarEtAl2021,SalazarLanzettiEtAl2019}. Finally, $D^\mathrm{rp}$ is not optimal w.r.t. the objective function of Problem~\ref{prob:rides}, but it is w.r.t. its relaxed version, enabling a polynomial-time computation.


==> Sections/NewModel.tex <==
% !TeX spellcheck = en_US

\section{Joint Optimization Method}


Congestion strongly influences travel
times. In this work we use the Bureau of Public Roads (BPR) function~\cite{BPR1964}, which can be expressed as $FBPR(x) = 1 + 0.15 · (f/C)^4$, with C representing the nominal capacity of the road, and $f$ the overall vehicles’ flow traversing it.
With the inclusion of the BPR function, the problems becomes non linear. Following~\cite{Wollenstein-BetechSalazarEtAl2021}, we approximate the BPR with a piece-wise two line function so that the problem remains linear and convex.


In this section we devise a new method to include the computation of matrix $D^\mathrm{rp}$ inside problem~\ref{prob:rides} so that they can be solved jointly. We recall that  $\sum_{n\in \cM} \gamma_{mn} \leq \alpha_m, \, \forall r_m \in \mathcal{R}$. In particular, the equality is never reached. For low demands $\sum_{n\in \cM} \gamma_{mn} << \alpha_m, \, \forall r_m \in \mathcal{R}$, meaning that many rides are not pooled together, while for very high demands, $\sum_{n\in \cM} \gamma_{mn} \rightarrow \alpha_m, \, \forall r_m \in \mathcal{R}$. For this reason, in a setting with road congestion, we assume there is a large set of travel requests, meaning that it is reasonable to assume $\sum_{n\in \cM} \gamma_{mn} \approx \alpha_m, \, \forall r_m \in \mathcal{R}$, i.e., almost every requests can be pooled with someone else~\cite{PaparellaPedrosoEtAl2023, Santi2014}.
By doing so, Problem~\ref{prob:rides} can be rewritten as follows:
\begin{prob}[Congested Ride-pooling Network Flow Problem]\label{prob:ridescongestion}
	Given a road graph $\cG$ and a set of travel requests $\cR$, the assignment matrix $\gamma$, the active vehicle flows $X$ and rebalancing flow $x^\mathrm{r}$ that minimize the cost in terms of overall travel time result from
	\begin{equation*}
		\begin{aligned}
			\min_{X,x^\mathrm{r},\gamma}\; &J(X,x^\mathrm{r}) = {t(X,x^\mathrm{r})^\top (X\mathds{1} + \rho x^\mathrm{r})} \\
			\mathrm{s.t. }\; & BX = D^\mathrm{rp}(\gamma) \\
			&B ( X \mathds{1}+ x^\mathrm{r} )= 0 \\
			& X, x^\mathrm{r} \geq 0 \\
			& D^\mathrm{rp}(\gamma) = \sum_{c,m,n} \gamma_{mn}^c D^{mn,c} \\
			%& \sum_c \gamma_{mn}^c = min(\alpha_m,\alpha_n) \\
			& \sum_{c,m} \gamma_{mn}^c = \alpha_n \\
			& \sum_{c,n} \gamma_{mn}^c = \alpha_m \\
			& \gamma_{mn}^c \geq 0
		\end{aligned}
	\end{equation*}
\end{prob}
\subsection{Discussion}
Few comments are in order. First, the key assumption is that there are enough travel requests so that everyone can be ride-pooled, as shown in the results in~\cite{PaparellaPedrosoEtAl2023, Santi2014}: For large number of travel requests, more than 95\% of the travel requests can be ride-pooled with waiting time lower than \unit[5]{min}; The percentage increases even further for waiting time in the order of \unit[10-15]{mins}. This is reflected in the implicit assumption that $P(\alpha_m,\alpha_n)=1$, which is a reasonable approximation for large $\alpha_m,\alpha_n$. To confirm numerically, by substituting $\alpha_m,\alpha_n = \unit[50]{requests/h}$ and $\bar{t}=\unit[10]{min}$ in~\eqref{eq:lem} the result is $0.9998$. Thus, in a congested setting with large number of travel requests and reasonable waiting time, this approximation seems plausible. 
Nevertheless, the set of travel requests can be downsized accordingly to take into account that not all the requests can actually be ride-pooled. 

Second, the matrices $D^{mn,c}$ are pre-computed, i.e., it is possible to either follow the path encoded in $D^{mn,c}$ or not. Thus, it is possible to eliminate a priori the paths that violate the maximum experienced delay without congestion. It is not possible to eliminate the paths that because of congestion violate the delay, but that would not violate it without congestion. Although there are no hard constraints on these violations, since the objective function minimizes the overall travel time, it would not be optimal to choose very congested and time-consuming paths, meaning that the joint optimization deals for the most part with the aforementioned problem. In addition, it would be possible to encode multiple paths per serving order, allowing to choose several options.

Last, the elements of $\gamma$ are continuous, so the overall problem remains linear (or non-linear, depending on the objective). 

==> Tools/acronyms.tex <==
\newcommand{\blueb}[1]{\textcolor{blue}{#1}}
\newcommand{\redb}[1]{\textcolor{red}{#1}}

\definecolor{lightblue}{rgb}{0.60784,0.76078,0.90196}
\definecolor{darkblue}{rgb}{0.26667,0.44706,0.76863}
\definecolor{lightgreen}{rgb}{0.66275,0.81569,0.55686}
\definecolor{darkgreen}{rgb}{0.43922,0.67843,0.27843}
\definecolor{orange}{rgb}{0.92941,0.49020,0.19216}
\definecolor{yellow}{rgb}{1.00000,0.75294,0.00000}
\definecolor{grey}{rgb}{0.64706,0.64706,0.64706}
\definecolor{purple}{rgb}{0.51373,0.23529,0.04706}
% a
\newacronym{abk:amod}{AMoD}{Autonomous Mobility-on-Demand}
\newacronym{abk:iamod}{I-AMoD}{intermodal \gls{abk:amod}}
% b
\newacronym{abk:bpr}{BPR}{the Bureau of Public Roads}
% c
\newacronym{abk:ca}{CA}{congestion-aware}
\newacronym{abk:cara}{CARS}{congestion-aware routing scheme}
\newacronym{abk:cepamods}{CEPAMoDS}{Convolutional Energy Predicting AMoD Scheduler}
\newacronym{abk:cs}{CS}{charging station}
% d
% e
% f
\newacronym{abk:ffcs}{FFCS}{free floating car sharing systems}
% g
\newacronym{abk:ghg}{GHG}{greenhouse gas}
% h
% i
% j
% k
\newacronym{abk:kpi}{KPIs}{Key Performance Indicators}
% l
% m
\newacronym{abk:mcfp}{MCFP}{multi-commodity flow problem}
\newacronym{abk:milp}{MILP}{mixed-integer linear program}
% n
% o
% p
% q
% r
% s
\newacronym{abk:spp}{SPP}{shortest path problem}
\newacronym{abk:kdspp}{k-dSPP}{k-disjoint \gls{abk:spp}}
\newacronym{abk:soc}{SoC}{state of charge}
% t
% u
% v
\newacronym{abk:vrp}{VRP}{vehicle routing problem}
\newacronym{abk:v2g}{V2G}{vehicle-to-grid}
% w
% x
% y
% z	
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Commands
% \newcommand{}{}
%-Large-Arabic-------------------------------------------------------------------------------
% A
%\newcommand{}{A}
\newcommand{\eqMatrix}{\mathbf{A}}
% B
%\newcommand{}{B}
% C
%\newcommand{}{C}
% D
%\newcommand{}{D}
\newcommand{\ineqMatrix}{\mathbf{D}}
% E
%\newcommand{}{E}
% F
%\newcommand{}{F}
\newcommand{\BPR}{F_\mathrm{BPR}}
% G
%\newcommand{}{G}
% H
%\newcommand{}{H}
% I
%\newcommand{}{I}
% J
%\newcommand{}{J}
% K
%\newcommand{}{K}
% L
%\newcommand{}{L}
% M
%\newcommand{}{M}
% N
%\newcommand{}{N}
% O
%\newcommand{}{O}
% P
%\newcommand{}{P}
\newcommand{\Pru}{P_\mathrm{rush}}
\newcommand{\Pch}{P_\mathrm{chill}}
% Q
%\newcommand{}{Q}
% R
%\newcommand{}{R}
% S
%\newcommand{}{S}
\newcommand{\source}{S_{o}}
\newcommand{\sink}{S_{d}}
% T
%\newcommand{}{T}
\newcommand{\resCost}{T^{\mathrm{c}}}
\newcommand{\resPred}{T^{\mathrm{p}}}
% U
%\newcommand{}{U}
% V
%\newcommand{}{V}
\newcommand{\vTime}{V_\mathrm{T}}
\newcommand{\vDistR}{V_\mathrm{D}}
\newcommand{\vDistS}{V_\mathrm{D,P}}
\newcommand{\vEnergy}{V_\mathrm{E}}
\newcommand{\vCO}{V_{\mathrm{CO}_2}}
\newcommand{\vQuadratic}{V_\mathrm{Q}}
% W
%\newcommand{}{W}
% X
%\newcommand{}{X}
% Y
%\newcommand{}{Y}
% Z
%\newcommand{}{Z}
%-Small-Arabic-------------------------------------------------------------------------------
% a
%\newcommand{}{a}
% b
%\newcommand{}{b}
\newcommand{\eqRHS}{\mathbf{b}}
% c
%\newcommand{}{c}
\newcommand{\capacity}{c}
\newcommand{\capacityRoad}{c^{\mathrm{R}}}
\newcommand{\capacityRoadTh}{c^{\mathrm{R,th}}}
\newcommand{\capacityPublic}{c^{\mathrm{P}}}
\newcommand{\cost}{J}
\newcommand{\costQ}{J_\mathrm{Q}}
\newcommand{\costM}{J_\mathrm{M}}
\newcommand{\costE}{J_{\mathrm{CO}_2}}
\newcommand{\transpCoeff}{\mathbf{c}^\top}
% d
%\newcommand{}{d}
\newcommand{\destination}{d}
\newcommand{\ineqRHS}{\mathbf{d}}
% e
%\newcommand{}{e}
\newcommand{\energyR}{e_{ij}}
\newcommand{\sC}{s_{\mathrm{CO}_2}}
\newcommand{\energyS}{e_{\mathrm{S},ij}}
\newcommand{\energySperpaxmile}{\bar{e}_{\mathrm{P}}}
% f
%\newcommand{}{f}
\newcommand{\flow}[2]{f_m\left(#1,#2\right)}
\newcommand{\flowTot}[2]{f\left(#1,#2\right)}
\newcommand{\flowzero}[2]{f_m\left(#1,#2\right)}
\newcommand{\flowReba}[2]{f_0\left(#1,#2\right)}
% g
%\newcommand{}{g}
% h
%\newcommand{}{h}
% i
%\newcommand{}{i}
% j
%\newcommand{}{j}
% k
%\newcommand{}{k}
% l
%\newcommand{}{l}
% m
%\newcommand{}{m}
% n
%\newcommand{}{n}
% o
%\newcommand{}{o}
\newcommand{\origin}{o}
% p
%\newcommand{}{p}
\newcommand{\route}{p}
\newcommand{\pSubway}{p_\mathrm{P}(i,j)}
\newcommand{\pRoad}{p_\mathrm{R}(i,j)}
\newcommand{\pOrigin}[1]{p_\mathrm{O}\left(#1\right)}
\newcommand{\pDest}[1]{p_\mathrm{D}\left(#1\right)}
% q
%\newcommand{}{q}
% r
%\newcommand{}{r}
\newcommand{\request}{r}
\newcommand{\weight}{r_\mathrm{E}}
% s
%\newcommand{}{s}
% t
%\newcommand{}{t}
\newcommand{\traveltime}{t}
\newcommand{\traveltimeNom}{t^N}
\newcommand{\traveltimezero}{t^0}
\newcommand{\tRoad}{\tau_\mathrm{R}(i,j)}
% u
%\newcommand{}{u}
\newcommand{\usageRoad}{u^\mathrm{R}}
% v
%\newcommand{}{v}
% w
%\newcommand{}{w}
% x
%\newcommand{}{x}
\newcommand{\decVec}{\mathbf{x}}
% y
%\newcommand{}{y}
% z
%\newcommand{}{z}
%-Large-Calligraphic-------------------------------------------------------------------------
% A
%\newcommand{}{\mathcal{A}}
\newcommand{\setOfArcs}{\mathcal{A}}
\newcommand{\setOfArcsRoad}{\mathcal{A}_{\mathrm{R}}}
\newcommand{\setOfArcsSubway}{\mathcal{A}_{\mathrm{P}}}
\newcommand{\setOfArcsPedestrian}{\mathcal{A}_{\mathrm{W}}}
\newcommand{\setOfArcsCommute}{\mathcal{A}_{\mathrm{C}}}
%\newcommand{\setOfArcsSP}{\mathcal{A}_{\mathrm{SP}}}
% B
%\newcommand{}{\mathcal{B}}
% C
%\newcommand{}{\mathcal{C}}
% D
%\newcommand{}{\mathcal{D}}
% E
%\newcommand{}{\mathcal{E}}
%\newcommand{\setOfArcs}{\mathcal{E}}
%\newcommand{\setOfArcsRoad}{\mathcal{E}_{\mathrm{R}}}
%\newcommand{\setOfArcsPublic}{\mathcal{E}_{\mathrm{P}}}
%\newcommand{\setOfArcsCommute}{\mathcal{E}_{\mathrm{C }}}
% F
%\newcommand{}{\mathcal{F}}
% G
%\newcommand{}{\mathcal{G}}
\newcommand{\Graph}{\mathcal{G}}
\newcommand{\GraphRoad}{\mathcal{G}_\mathrm{R}}
\newcommand{\GraphSubway}{\mathcal{G}_\mathrm{P}}
\newcommand{\GraphPedestrian}{\mathcal{G}_\mathrm{W}}
% H
%\newcommand{}{\mathcal{H}}
% I
%\newcommand{}{\mathcal{I}}
% J
%\newcommand{}{\mathcal{J}}
% K
%\newcommand{}{\mathcal{K}}
\newcommand{\setOfModes}{\mathcal{K}}
% L
%\newcommand{}{\mathcal{L}}
% M
%\newcommand{}{\mathcal{M}}
\newcommand{\setOfRequestsNumber}{\mathcal{M}}
% N
%\newcommand{}{\mathcal{N}}
% O
%\newcommand{}{\mathcal{O}}
% P
%\newcommand{}{\mathcal{P}}
\newcommand{\pathSet}{\mathcal{P}}
% Q
%\newcommand{}{\mathcal{Q}}
% R
%\newcommand{}{\mathcal{R}}
\newcommand{\setOfRequests}{\mathcal{R}}
% S
%\newcommand{}{\mathcal{S}}
\newcommand{\subSet}{\mathcal{S}}
% T
%\newcommand{}{\mathcal{T}}
% U
%\newcommand{}{\mathcal{U}}
% V
%\newcommand{}{\mathcal{V}}
\newcommand{\setOfVertices}{\mathcal{V}}
\newcommand{\setOfVerticesRoad}{\mathcal{V}_{\mathrm{R}}}
\newcommand{\setOfVerticesSubway}{\mathcal{V}_{\mathrm{P}}}
\newcommand{\setOfVerticesPedestrian}{\mathcal{V}_{\mathrm{W}}}
% W
%\newcommand{}{\mathcal{W}}
% X
%\newcommand{}{\mathcal{X}}
% Y
%\newcommand{}{\mathcal{Y}}
% Z
%\newcommand{}{\mathcal{Z}}
%-Large-Scr-------------------------------------------------------------------------
% A
%\newcommand{}{\mathscr{A}}
\newcommand{\setOfMultiArcs}{\mathscr{A}}
% B
%\newcommand{}{\mathscr{B}}
% C
%\newcommand{}{\mathscr{C}}
% D
%\newcommand{}{\mathscr{D}}
% E
%\newcommand{}{\mathscr{E}}
% F
%\newcommand{}{\mathscr{F}}
% G
%\newcommand{}{\mathscr{G}}
\newcommand{\multigraph}{\mathscr{G}}
\newcommand{\multigraphC}{\mathscr{G}'}
% H
%\newcommand{}{\mathscr{H}}
% I
%\newcommand{}{\mathscr{I}}
% J
%\newcommand{}{\mathscr{J}}
% K
%\newcommand{}{\mathscr{K}}
% L
%\newcommand{}{\mathscr{L}}
% M
%\newcommand{}{\mathscr{M}}
% N
%\newcommand{}{\mathscr{N}}
% O
%\newcommand{}{\mathscr{O}}
% P
%\newcommand{}{\mathscr{P}}
\newcommand{\setOfArcsIndex}{\mathscr{P}}
% Q
%\newcommand{}{\mathscr{Q}}
% R
%\newcommand{}{\mathscr{R}}
% S
%\newcommand{}{\mathscr{S}}
% T
%\newcommand{}{\mathscr{T}}
% U
%\newcommand{}{\mathscr{U}}
% V
%\newcommand{}{\mathscr{V}}
% W
%\newcommand{}{\mathscr{W}}
% X
\newcommand{\decvecSet}{\mathcal{X}}
% Y
%\newcommand{}{\mathscr{Y}}
% Z
%\newcommand{}{\mathscr{Z}}
\newcommand{\setOfMultiarcIndex}{\mathscr{Z}}
%-Large-Greek--------------------------------------------------------------------------------
% Alpha
%\newcommand{}{A}
% Beta
%\newcommand{}{B}
% Gamma
%\newcommand{}{\Gamma}\\
\newcommand{\neighborOne}{\Gamma}
% Delta
%\newcommand{}{\Delta}
% Epsilon
%\newcommand{}{E}
% Zeta
%\newcommand{}{Z}
% Eta
%\newcommand{}{H}
% Theta
%\newcommand{}{\Theta}
% Iota
%\newcommand{}{I}
% Kappa
%\newcommand{}{K}
% Lambda
%\newcommand{}{\Lambda}
% Mu
%\newcommand{}{M}
% Nu
%\newcommand{}{N}
% Xi
%\newcommand{}{\Xi}
% Omicron
%\newcommand{}{O}
% Pi
%\newcommand{}{\Pi}
% Rho
%\newcommand{}{P}
% Sigma
%\newcommand{}{\Sigma}
% Tau
%\newcommand{}{T}
% Upsilon
%\newcommand{}{\Upsilon}
% Phi
%\newcommand{}{\Phi}
% Chi
%\newcommand{}{X}
% Psi
%\newcommand{}{\Psi}
% Omega
%\newcommand{}{\Omega}
%-Small-Greek--------------------------------------------------------------------------------
% alpha
%\newcommand{}{\alpha}
\newcommand{\requestrate}{\alpha}
% beta
%\newcommand{}{\beta}
% gamma
%\newcommand{}{\gamma}
% delta
%\newcommand{}{\delta}
\newcommand{\cutsetSucc}[1]{\delta^{\text{+}}\left(#1\right)}
\newcommand{\cutsetPred}[1]{\delta^{\text{-}}\left(#1\right)}
% epsilon
%\newcommand{\slack}{\varepsilon}
\newcommand{\slack}[2]{\varepsilon\left(#1,#2\right)}
% zeta
%\newcommand{}{\zeta}
% eta
%\newcommand{}{\eta}
% theta
%\newcommand{}{\vartheta}
% iota
%\newcommand{}{\iota}
\newcommand{\iteration}{\iota}
% kappa
%\newcommand{}{\kappa}
% lambda
%\newcommand{}{\lambda}
\newcommand{\lgeq}{\mathbf{\lambda}}
\newcommand{\dualEq}{\lambda_{ij}}
\newcommand{\dualCust}{\lambda_\mathrm{C}}
\newcommand{\dualVeh}{\lambda_\mathrm{R}}
\newcommand{\dualCustTilde}{\tilde{\lambda}_\mathrm{C}}
\newcommand{\dualVehTilde}{\tilde{\lambda}_\mathrm{R}}
% mu
%\newcommand{}{\mu}
\newcommand{\dualCR}{\mu_\mathrm{cR}}
\newcommand{\lgineq}{\mathbf{\mu}}
\newcommand{\dualIneq}{\mu}
\newcommand{\dualcR}{\mu_\mathrm{cR}}
\newcommand{\dualcS}{\mu_\mathrm{cP}}
% nu
%\newcommand{}{\nu}
% xi
%\newcommand{}{\xi}
% omicron
%\newcommand{}{o}
% pi
%\newcommand{}{\pi}
% rho
%\newcommand{}{\rho}
% sigma
%\newcommand{}{\sigma}
% tau
%\newcommand{}{\tau}
% upsilon
%\newcommand{}{\upsilon}
% phi
%\newcommand{}{\phi}
% chi
%\newcommand{}{\chi}
% psi
%\newcommand{}{\psi}
% omega
%\newcommand{}{\omega}
%-Other-------------------------------------------------------------------
\newcommand{\arc}{(i,j)}
\newcommand{\multiarc}{(i,j,z)}
\newcommand{\bool}[1]{\mathds{1}_{#1}}
